Critical discussion of Tomboulis's approach to the confinement problem

The approach to the confinement problem proposed by E.T. Tomboulis is analyzed critically. We point out some problems and discuss the chances of producing a proof by using his strategy.

==> conclusions <==
\overlays{4}{
\begin{slide}{V. Can the problems be fixed?}
\begin{itemstep}

\item
Choice of $\g {r}$ very subtle. Have to ensure {\B interpolation 
parameters} $\g {\alpha^*}$ bounded away from 1 {\B and} convergence of 
MKT to strong coupling FP.
\vglue5mm
\item
$\g {U(1)}$ instructive: for $\g {r=1}$ such $\g {\alpha^*}$ {\red cannot}
exist; for $\g {r<1}$ it may exist, but does not imply confinement.
\vglue5mm
\item
Migdal-Kadanoff strategy {\B unlikely} to succeed: predicts permanent 
confinement for {\B all} $\g {SU(N)}$ and $\g {U(N)}$ in $\g {D=4}$.
 

\end{itemstep}
\end{slide}}



==> fundamental <==
\overlays{3}{
\begin{slide}{}
\fromSlide{1}{\vglue-5mm 
{\it \Large\B III. The Fundamental Issue}\\
\vglue2mm
{\B Fact:} In $\g {D=4}$ MK RG flows to strong coupling fixed point 
-- abelian or nonabelian.}
\fromSlide{2}{\vglue5mm
Stated by {\red Wilson 1976, Jos\'e et al 1977}\\
(Numerically: {\red E.S.\& U. Wolff 1983})\\
\vglue5mm
Proof: {\red K.R. Ito 1985}}
\vglue5mm
\fromSlide{3}{
{\B Consequence:} Comparison argument with MK RG has to {\red fail} for 
$\g {U(1)}$.

{\B Any such argument} that does not explicitly make use of nonabelian 
nature has to {\B fail}.}

\end{slide}}


==> intro <==
\overlays{5}{
\begin{slide}{I. Historical Remarks}
%\vglue-10mm
\fromSlide{1}{
{\B Confinement hot issue end of 70's, early 80's}}
\fromSlide{2}{\vglue4mm
Center vortices as key ingredients: {\red Yoneya 1977, 't Hooft 1979, 
Mack\&Petkova 1980}}
\fromSlide{3}{\vglue4mm
't Hooft's string tension sufficient for confinement: {\red Borgs\&Seiler 
1983, Tomboulis\&Yaffe 1985}}
\fromSlide{4}{\vglue4mm
MK-approximate Renormalization Group: 
{\red Migdal 1975; Kadanoff 1976; Jos\'e, Kadanoff, Kirkpatrick, Nelson 
1977}}
\fromSlide{5}{\vglue4mm
Rigorous results on MK RG: 
{\red Ito 1985, M\"uller\&Schiemann 1988}}

\end{slide}}

\overlays{5}{
\begin{slide}{}
\vglue-10mm
\fromSlide{1}{
{\B Charming idea} ({\red E.~T.~Tomboulis 1982}):\\ Compare exact RG to MK 
RG by exact inequalities to show permanent confinement \`a la \t Hooft.} 
\fromSlide{2}{\vglue5mm
{\B Details missing.}}
\fromSlide{3}{\vglue5mm
{\B Problems discovered} ({\red Mack, Seiler\&Wolff, Ito}).} 
\fromSlide{4}{\vglue5mm
1987-2002: {\red A. Patrascioiu and E.~S.} try to show absence of 
permanent confinement. Others, among them {\red K.~R.~Ito} work on proof 
of confinement. 
{\B Issue unsettled.}}
\fromSlide{5}{\vglue5mm
2007: {\red Tomboulis} revives old idea.} 

\end{slide}}



==> macros <==

% Definitions and abbreviations

\font\sixrm=cmr6
\newcommand{\nonum}{\nonumber \\[1.5mm]}
\newcommand{\bspace}{\makebox[2cm]{ }}
\newcommand{\sspace}{\makebox[1cm]{ }}
\newcommand{\nspace}{\!\!\!\!\!\!\!\!\!\!}

%Environments
\newtheorem{theorem}{Theorem}


%Blackboard boldface
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\bR}{\mathbb{R}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\T}{\mathbb{T}}
\renewcommand{\P}{\mathbb{P}}
\renewcommand{\H}{\mathbb{H}}
\newcommand{\1}{\mbox{1\hspace{-.4ex}I}}

%colors
%\newcommand{\g}{\PineGreen}
\newcommand{\g}{\OliveGreen}
%\newcommand{\g}{\green}
%\newcommand{\g}{\ForestGreen}
\newcommand{\B}{\blue}

%greek letters
\newcommand{\om}{\omega}

%\script letters
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}

% Roman letters in math formulae

\def\rmd{{\rm d}}
\def\rmD{{\rm D}}
\def\rme{{\rm e}}
\def\rmO{{\rm O}}
\def\bfx{{\bf x}}
\def\bfy{{\bf y}}
\def\bfr{{\bf r}}
\def\bfz{{\bf z}}
\def\la{\langle}
\def\ra{\rangle}
\def\tr{{\rm tr}}

% Real and integer numbers

\def\rz{\rm I\kern-.2emR}
\def\gz{{\rm Z\kern-.48em Z}}
\def\Im{{\rm Im}\,}
\def\Re{{\rm Re}\,}

% Special relations and symbols

\def\up{\uparrow}
\def\defeq{\mathrel{\mathop=^{\rm def}}}
\def\proof{\noindent{\sl Proof:}\kern0.6em}
\def\endproof{\hskip0.6em plus0.1em minus0.1em
\setbox0=\null\ht0=5.4pt\dp0=1pt\wd0=5.3pt
\vbox{\hrule height0.8pt
\hbox{\vrule width0.8pt\box0\vrule width0.8pt}
\hrule height0.8pt}}
\def\frac#1#2{\hbox{$#1\over#2$}}
\def\dual{\mathstrut^*\kern-0.1em}
\def\mod{\;\hbox{\rm mod}\;}
\def\ring{\mathaccent"7017}
\def\lvec#1{\setbox0=\hbox{$#1$}
    \setbox1=\hbox{$\scriptstyle\leftarrow$}
    #1\kern-\wd0\smash{
    \raise\ht0\hbox{$\raise1pt\hbox{$\scriptstyle\leftarrow$}$}}
    \kern-\wd1\kern\wd0}
\def\rvec#1{\setbox0=\hbox{$#1$}
    \setbox1=\hbox{$\scriptstyle\rightarrow$}
    #1\kern-\wd0\smash{
    \raise\ht0\hbox{$\raise1pt\hbox{$\scriptstyle\rightarrow$}$}}
    \kern-\wd1\kern\wd0}

% Lattice derivatives

\def\nab#1{{\nabla_{#1}}}
\def\nabstar#1{\nabla\kern-0.5pt\smash{\raise 4.5pt\hbox{$\ast$}}
               \kern-4.5pt_{#1}}
\def\drv#1{{\partial_{#1}}}
\def\drvstar#1{\partial\kern-0.5pt\smash{\raise 4.5pt\hbox{$\ast$}}
               \kern-5.0pt_{#1}}


% Units

\def\MeV{{\rm MeV}}
\def\GeV{{\rm GeV}}
\def\TeV{{\rm TeV}}
\def\fm{{\rm fm}}

\def\fpi{F_{\pi}}

% Constants

\def\euler{\gamma_{\rm E}}

% Improvement coefficients

\def\be{\begin{displaymath}}
\def\ee{\end{displaymath}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}


==> strategy <==
\overlays{2}{
\begin{slide}{}\vglue-10mm
{\Large \B II. Sketch of Tomboulis' Strategy}
\vglue4mm
\fromSlide{1}{
$\g {SU(2)}$ Yang-Mills on lattice, want to show {\B spreading} of 
{\B central magnetic flux} in $\g {L_1\times L_2\times L_3\times L_4}$ 
torus: 
\be
\g {\frac{Z_\Lambda^{(-)}}{Z_\Lambda}\ge \exp\left[\sigma\, L_3 L_4 
e^{-L_1 L_2}\right]
}
\ee
where $\g {Z_\Lambda^{(-)}}$ has twisted b.c. in the (12)-direction.}

\fromSlide{2}{
This is supposed to follow from 
\be
\g {\frac{Z_\Lambda^{(-)}}{Z_\Lambda}\ge 
\frac{Z^{(-)}_{MKT}(n)}{Z_{MKT}(n)}
}
\ee
Here $\g {Z_{MKT}(n)}$, $\g {Z^{(-)}_{MKT}(n)}$ partition 
functions under $\g n$-fold iteration of the 
{\red Migdal-Kadanoff-Tomboulis} decimation.}


\end{slide}}

\overlays{3}{
\begin{slide}{}
\fromSlide{1}{
{\red Assume:} Inequality holds {\B and} MKT iteration eventually leads to 
strong coupling regime $\Longrightarrow$  
\begin{itemize}
\item
{\B spreading of magnetic flux} 
\item
 {\B electric flux string formation}
\end{itemize}}
\fromSlide{2}{\vglue5mm
{\B Question:} True for MKT RG in $\g {D=4}$? Depends on a parameter 
$\g {r=1-\epsilon}$.}
\fromSlide{3}{ 
\vglue5mm
{\red Caution!} $\g {r<1}$ effectively increases dimension.}

\end{slide}}


==> technical <==
\overlays{2}{
\begin{slide} { IV. Technical Issues}
%\vspace{-0.1cm}
\fromSlide{1}{
\begin{itemize}
\item 
The parameter $\g {r}$:

{\B Character expansion} of plaquette coupling
\be \g{
f(U)\equiv \exp A_p(U)=
F_0\left[1+\sum_{j\neq0}(2j+1)c_j(\beta)\chi_j(U)\right]\,.
}\ee
}
\fromSlide{2}{\vglue4mm
MK{\red T} decimation: alternate raising coupling function 
to power $\g {b^2=4}$ and Fourier coefficients $\g {c_j}$ 
to power $\g {b^2{\red r}=4{\red r}}$.
}
\end{itemize}
\end{slide}}

\overlays{2}{
\begin{slide}{}
\fromSlide{1}{\vglue-8mm
Concretely
\be \g{
f^{(n)}(U)\mapsto \frac{f^{(n)}(U)^4}{\int f^{(n)}(U)^4 dU}\equiv 
g^{(n)}(U)
}\ee
\vspace{-5mm}
\be \g{
g^{(n)}(U)=1+\sum_{j>0} (2j+1)c_j(n) \chi_j(U)
}\ee
\be\g{
f^{(n+1)}(U)=1+\sum_{j>0} (2j+1)c_j(n)^{4{\red r}} \chi_j(U)
}\ee
}
\fromSlide{2}{
{\B Note:} Exponent $\g {4}$ is really $\g {2^{D-2}}$ for $\g {D=4}$ , so 
introducing $\g {r<1}$ is similar to reducing $\g {D}$.}
\end{slide}}

\begin{slide}{}
 For $\g {r<1}$ {\B phase transition}:
\begin{figure}[htb]
\includegraphics[width=.45\columnwidth]{mktc4.80.eps}
\includegraphics[width=.45\columnwidth]{mktc4.79.eps}
\label{plot}
\end{figure}
\vglue-5mm
\hglue15mm$\g {\beta=4.80}$\hglue35mm $\g {\beta=4.79}$\\
Evolution of $\g {c_j/c_0}$ under MKT RG with $\g {r=0.9}$. 

\end{slide}

\begin{slide}{}

\begin{itemize}

\item 
{\B Existence} of common interpolation parameter $\g {\alpha^*}$ for both 
twisted and untwisted partition functions?


{\red Crucial point} in T.'s argument: 
\be\g{
\exists\; 0<\alpha^*(n)\le 1-\delta \quad{\rm such\; that}
}\ee
\be\g{
\frac{Z_{\Lambda}^{(-)} (\{c_{j}\})} {Z_{\Lambda}(\{c_{j}\})}
=\frac{Z_{\Lambda}^{(-)} (\{\alpha^*(n)c_{j}(n)\})}
      {Z_{\Lambda} (\{\alpha^*(n)c_{j}(n)\})} 
}\ee
Essential: $\g {\alpha^*}$ bounded {\B uniformly} away from $\g {1}$,\\
i.e. $\g {\delta >0}$ independent of $\g {n}$.

\end{itemize}

\end{slide}

\overlays{5}{
\begin{slide}{}
\vspace{-10mm}
\fromSlide{1}{
Argument based on {\B implicit function theorem:} Flawed.}
\fromSlide{2}{
T. introduces function  $\g{\Psi_t(\lambda,t)}$ in terms of 
interpolated partition functions and requires
\be\g{
\Psi_t(\lambda,t)=0\,.
}\ee
}
\fromSlide{3}{
Solved for $\g {\lambda=0}$ by $\g {t=t_0}$. Need solution up to 
$\g {\lambda=1}.$}
\fromSlide{4}{
{\B \,\,Claim:} follows from 
\be\g{
\frac{\partial}{\partial t}\Psi_t(\lambda,t)\neq 0\,.
}\ee
}
\fromSlide{5}{
{\B Counterexample} (in thesis of {\red Takuya Kanazawa}):
\be\g{
\Psi_t(\lambda,t)\equiv e^{-t}-1+2\lambda\,.
}\ee
{\B \, More is needed.}}
%\end{itemize}
\end{slide}}


